Enhanced Fine-Tuning of Lightweight Domain-Specific Q&A Model Based on Large Language Models

Large language models (LLMs) excel at general question-answering (Q&A) but often fall short in specialized domains due to a lack of domain-specific knowledge. Commercial companies face the dual challenges of privacy protection and resource constraints when involving LLMs for fine-tuning. This paper propose a novel framework, Self-Evolution, designed to address these issues by leveraging lightweight open-source LLMs through multiple iterative fine-tuning rounds. To enhance the efficiency of iterative fine-tuning, Self-Evolution employ a strategy that filters and reinforces the knowledge with higher value during the iterative process. We employed Self-Evolution on Qwen1.5-7B-Chat using 4,000 documents containing rich domain knowledge from China Mobile, achieving a performance score 174% higher on domain-specific question-answering evaluations than Qwen1.5-7B-Chat and even 22% higher than Qwen1.5-72B-Chat. Self-Evolution has been deployed in China Mobile's daily operation and maintenance for 117 days, and it improves the efficiency of locating alarms, fixing problems, and finding related reports, with an average efficiency improvement of over 18.6%. In addition, we release Self-Evolution framework code in https://github.com/Zero-Pointer/Self-Evolution.

==> reference.tex <==
@article{guo2023owl,
  title={Owl: A large language model for it operations},
  author={Guo, Hongcheng and Yang, Jian and Liu, Jiaheng and Yang, Liqun and Chai, Linzheng and Bai, Jiaqi and Peng, Junran and Hu, Xiaorong and Chen, Chao and Zhang, Dongfeng and others},
  journal={arXiv preprint arXiv:2309.09298},
  year={2023}
}
@inproceedings{jin2023assess,
  title={Assess and summarize: Improve outage understanding with large language models},
  author={Jin, Pengxiang and Zhang, Shenglin and Ma, Minghua and Li, Haozhe and Kang, Yu and Li, Liqun and Liu, Yudong and Qiao, Bo and Zhang, Chaoyun and Zhao, Pu and others},
  booktitle={Proceedings of the 31st ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={1657--1668},
  year={2023}
}
@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}
@article{raffel2020exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={Journal of machine learning research},
  volume={21},
  number={140},
  pages={1--67},
  year={2020}
}
@article{ouyang2022training,
  title={Training language models to follow instructions with human feedback},
  author={Ouyang, Long and Wu, Jeffrey and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and others},
  journal={Advances in neural information processing systems},
  volume={35},
  pages={27730--27744},
  year={2022}
}
@article{wei2021finetuned,
  title={Finetuned language models are zero-shot learners},
  author={Wei, Jason and Bosma, Maarten and Zhao, Vincent Y and Guu, Kelvin and Yu, Adams Wei and Lester, Brian and Du, Nan and Dai, Andrew M and Le, Quoc V},
  journal={arXiv preprint arXiv:2109.01652},
  year={2021}
}
@inproceedings{longpre2023flan,
  title={The flan collection: Designing data and methods for effective instruction tuning},
  author={Longpre, Shayne and Hou, Le and Vu, Tu and Webson, Albert and Chung, Hyung Won and Tay, Yi and Zhou, Denny and Le, Quoc V and Zoph, Barret and Wei, Jason and others},
  booktitle={International Conference on Machine Learning},
  pages={22631--22648},
  year={2023},
  organization={PMLR}
}
@article{sanh2021multitask,
  title={Multitask prompted training enables zero-shot task generalization},
  author={Sanh, Victor and Webson, Albert and Raffel, Colin and Bach, Stephen H and Sutawika, Lintang and Alyafeai, Zaid and Chaffin, Antoine and Stiegler, Arnaud and Scao, Teven Le and Raja, Arun and others},
  journal={arXiv preprint arXiv:2110.08207},
  year={2021}
}
@article{chung2022scaling,
  title={Scaling Instruction-Finetuned Language Models},
  author={Chung, Hyung Won and Hou, Le and Longpre, Shayne and Zoph, Barret and Tay, Yi and Fedus, William and Li, Yunxuan and Wang, Xuezhi and Dehghani, Mostafa and Brahma, Siddhartha and others},
  journal={arXiv e-prints},
  pages={arXiv--2210},
  year={2022}
}
@article{peng2023instruction,
  title={Instruction tuning with gpt-4},
  author={Peng, Baolin and Li, Chunyuan and He, Pengcheng and Galley, Michel and Gao, Jianfeng},
  journal={arXiv preprint arXiv:2304.03277},
  year={2023}
}
@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}
@misc{taori2023stanford,
  title={Stanford alpaca: An instruction-following llama model},
  author={Taori, Rohan and Gulrajani, Ishaan and Zhang, Tianyi and Dubois, Yann and Li, Xuechen and Guestrin, Carlos and Liang, Percy and Hashimoto, Tatsunori B},
  year={2023}
}
@article{xu2023wizardlm,
  title={Wizardlm: Empowering large language models to follow complex instructions},
  author={Xu, Can and Sun, Qingfeng and Zheng, Kai and Geng, Xiubo and Zhao, Pu and Feng, Jiazhan and Tao, Chongyang and Jiang, Daxin},
  journal={arXiv preprint arXiv:2304.12244},
  year={2023}
}
@misc{vicuna2023,
    title = {Vicuna: An Open-Source Chatbot Impressing GPT-4 with 90\%* ChatGPT Quality},
    url = {https://lmsys.org/blog/2023-03-30-vicuna/},
    author = {Chiang, Wei-Lin and Li, Zhuohan and Lin, Zi and Sheng, Ying and Wu, Zhanghao and Zhang, Hao and Zheng, Lianmin and Zhuang, Siyuan and Zhuang, Yonghao and Gonzalez, Joseph E. and Stoica, Ion and Xing, Eric P.},
    month = {March},
    year = {2023}
}
@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
}
@article{li2022explanations,
  title={Explanations from large language models make small reasoners better},
  author={Li, Shiyang and Chen, Jianshu and Shen, Yelong and Chen, Zhiyu and Zhang, Xinlu and Li, Zekun and Wang, Hong and Qian, Jing and Peng, Baolin and Mao, Yi and others},
  journal={arXiv preprint arXiv:2210.06726},
  year={2022}
}
@Misc{sharegpt2023,
    title = {ShareGPT},
    url = {https://sharegpt.com/},
    author = {ShareGPT},
    year = {2023}
}
@article{wang2022self,
  title={Self-instruct: Aligning language models with self-generated instructions},
  author={Wang, Yizhong and Kordi, Yeganeh and Mishra, Swaroop and Liu, Alisa and Smith, Noah A and Khashabi, Daniel and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:2212.10560},
  year={2022}
}
@article{sun2024principle,
  title={Principle-driven self-alignment of language models from scratch with minimal human supervision},
  author={Sun, Zhiqing and Shen, Yikang and Zhou, Qinhong and Zhang, Hongxin and Chen, Zhenfang and Cox, David and Yang, Yiming and Gan, Chuang},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}
@article{xu2023baize,
  title={Baize: An open-source chat model with parameter-efficient tuning on self-chat data},
  author={Xu, Canwen and Guo, Daya and Duan, Nan and McAuley, Julian},
  journal={arXiv preprint arXiv:2304.01196},
  year={2023}
}
@article{touvron2023llama,
  title={Llama 2: Open foundation and fine-tuned chat models},
  author={Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert, Peter and Almahairi, Amjad and Babaei, Yasmine and Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal and Bhosale, Shruti and others},
  journal={arXiv preprint arXiv:2307.09288},
  year={2023}
}
@article{sun2023salmon,
  title={Salmon: Self-alignment with principle-following reward models},
  author={Sun, Zhiqing and Shen, Yikang and Zhang, Hongxin and Zhou, Qinhong and Chen, Zhenfang and Cox, David and Yang, Yiming and Gan, Chuang},
  journal={arXiv preprint arXiv:2310.05910},
  year={2023}
}
@article{tsang2005core,
  title={Core vector machines: Fast SVM training on very large data sets.},
  author={Tsang, Ivor W and Kwok, James T and Cheung, Pak-Ming and Cristianini, Nello},
  journal={Journal of Machine Learning Research},
  volume={6},
  number={4},
  year={2005}
}
@inproceedings{har2005smaller,
  title={Smaller coresets for k-median and k-means clustering},
  author={Har-Peled, Sariel and Kushal, Akash},
  booktitle={Proceedings of the twenty-first annual symposium on Computational geometry},
  pages={126--134},
  year={2005}
}
@article{munteanu2018coresets,
  title={On coresets for logistic regression},
  author={Munteanu, Alexander and Schwiegelshohn, Chris and Sohler, Christian and Woodruff, David},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}
@article{zhou2024lima,
  title={Lima: Less is more for alignment},
  author={Zhou, Chunting and Liu, Pengfei and Xu, Puxin and Iyer, Srinivasan and Sun, Jiao and Mao, Yuning and Ma, Xuezhe and Efrat, Avia and Yu, Ping and Yu, Lili and others},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}
@inproceedings{mindermann2022prioritized,
  title={Prioritized training on points that are learnable, worth learning, and not yet learnt},
  author={Mindermann, S{\"o}ren and Brauner, Jan M and Razzak, Muhammed T and Sharma, Mrinank and Kirsch, Andreas and Xu, Winnie and H{\"o}ltgen, Benedikt and Gomez, Aidan N and Morisot, Adrien and Farquhar, Sebastian and others},
  booktitle={International Conference on Machine Learning},
  pages={15630--15649},
  year={2022},
  organization={PMLR}
}
@article{cao2023instruction,
  title={Instruction mining: High-quality instruction data selection for large language models},
  author={Cao, Yihan and Kang, Yanbin and Sun, Lichao},
  journal={arXiv preprint arXiv:2307.06290},
  year={2023}
}
@article{chen2023alpagasus,
  title={Alpagasus: Training a better alpaca with fewer data},
  author={Chen, Lichang and Li, Shiyang and Yan, Jun and Wang, Hai and Gunaratna, Kalpa and Yadav, Vikas and Tang, Zheng and Srinivasan, Vijay and Zhou, Tianyi and Huang, Heng and others},
  journal={arXiv preprint arXiv:2307.08701},
  year={2023}
}
@article{toneva2018empirical,
  title={An empirical study of example forgetting during deep neural network learning},
  author={Toneva, Mariya and Sordoni, Alessandro and Combes, Remi Tachet des and Trischler, Adam and Bengio, Yoshua and Gordon, Geoffrey J},
  journal={arXiv preprint arXiv:1812.05159},
  year={2018}
}
@article{paul2021deep,
  title={Deep learning on a data diet: Finding important examples early in training},
  author={Paul, Mansheej and Ganguli, Surya and Dziugaite, Gintare Karolina},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={20596--20607},
  year={2021}
}
@article{li2023quantity,
  title={From quantity to quality: Boosting llm performance with self-guided data selection for instruction tuning},
  author={Li, Ming and Zhang, Yong and Li, Zhitao and Chen, Jiuhai and Chen, Lichang and Cheng, Ning and Wang, Jianzong and Zhou, Tianyi and Xiao, Jing},
  journal={arXiv preprint arXiv:2308.12032},
  year={2023}
}
@article{bai2023qwen,
  title={Qwen technical report},
  author={Bai, Jinze and Bai, Shuai and Chu, Yunfei and Cui, Zeyu and Dang, Kai and Deng, Xiaodong and Fan, Yang and Ge, Wenbin and Han, Yu and Huang, Fei and others},
  journal={arXiv preprint arXiv:2309.16609},
  year={2023}
}
@article{zhang2023self,
  title={Self-qa: Unsupervised knowledge guided language model alignment},
  author={Zhang, Xuanyu and Yang, Qing},
  journal={arXiv preprint arXiv:2305.11952},
  year={2023}
}
@article{huang2023survey,
  title={A survey on hallucination in large language models: Principles, taxonomy, challenges, and open questions},
  author={Huang, Lei and Yu, Weijiang and Ma, Weitao and Zhong, Weihong and Feng, Zhangyin and Wang, Haotian and Chen, Qianglong and Peng, Weihua and Feng, Xiaocheng and Qin, Bing and others},
  journal={arXiv preprint arXiv:2311.05232},
  year={2023}
}
@article{liu2023pre,
  title={Pre-train, prompt, and predict: A systematic survey of prompting methods in natural language processing},
  author={Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
  journal={ACM Computing Surveys},
  volume={55},
  number={9},
  pages={1--35},
  year={2023},
  publisher={ACM New York, NY}
}
@article{hu2021lora,
  title={Lora: Low-rank adaptation of large language models},
  author={Hu, Edward J and Shen, Yelong and Wallis, Phillip and Allen-Zhu, Zeyuan and Li, Yuanzhi and Wang, Shean and Wang, Lu and Chen, Weizhu},
  journal={arXiv preprint arXiv:2106.09685},
  year={2021}
}
@article{gekhman2024does,
  title={Does Fine-Tuning LLMs on New Knowledge Encourage Hallucinations?},
  author={Gekhman, Zorik and Yona, Gal and Aharoni, Roee and Eyal, Matan and Feder, Amir and Reichart, Roi and Herzig, Jonathan},
  journal={arXiv preprint arXiv:2405.05904},
  year={2024}
}
@article{peiartificial,
  title={Artificial intelligence for IT operations in era of large language model},
  author={PEI, D and ZHANG, SL and SUN, YQ and others},
  journal={ZTE technology journal},
  year={2024}
}
@inproceedings{papineni2002bleu,
  title={Bleu: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting of the Association for Computational Linguistics},
  pages={311--318},
  year={2002}
}
@inproceedings{chen2024auto,
author = {Chen, Yinfang and Xie, Huaibing and Ma, Minghua and Kang, Yu and Gao, Xin and Shi, Liu and Cao, Yunjie and Gao, Xuedong and Fan, Hao and Wen, Ming and Zeng, Jun and Ghosh, Supriyo and Zhang, Xuchao and Zhang, Chaoyun and Lin, Qingwei and Rajmohan, Saravan and Zhang, Dongmei and Xu, Tianyin},
title = {Automatic Root Cause Analysis via Large Language Models for Cloud Incidents},
year = {2024},
isbn = {9798400704376},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3627703.3629553},
doi = {10.1145/3627703.3629553},
booktitle = {Proceedings of the Nineteenth European Conference on Computer Systems},
pages = {674–688},
numpages = {15},
keywords = {Cloud Systems, Large Language Models, Root Cause Analysis},
location = {Athens, Greece},
series = {EuroSys '24}
}
@inproceedings{guo2024owl,
title={{OWL}: A Large Language Model for {IT} Operations},
author={Hongcheng Guo and Jian Yang and Jiaheng Liu and Liqun Yang and Linzheng Chai and Jiaqi Bai and Junran Peng and Xiaorong Hu and Chao Chen and Dongfeng Zhang and xu Shi and Tieqiao Zheng and liangfan zheng and Bo Zhang and Ke Xu and Zhoujun Li},
booktitle={The Twelfth International Conference on Learning Representations},
year={2024},
url={https://openreview.net/forum?id=SZOQ9RKYJu}
}
@article{cui2023chatlaw,
  title={Chatlaw: Open-source legal large language model with integrated external knowledge bases},
  author={Cui, Jiaxi and Li, Zongjian and Yan, Yang and Chen, Bohua and Yuan, Li},
  journal={arXiv preprint arXiv:2306.16092},
  year={2023}
}

==> tabs/authors.tex <==
% \author{
% \IEEEauthorblockN{1\textsuperscript{st} Shenglin Zhang}
% \IEEEauthorblockA{\textit{College of Software} \\
% \textit{Nankai University}\\
% Tianjin, China \\
% zhangsl@nankai.edu.cn}
% \and
% \IEEEauthorblockN{2\textsuperscript{nd} Pengtian Zhu}
% \IEEEauthorblockA{\textit{College of Software} \\
% \textit{Nankai University}\\
% Tianjin, China \\
% zpt@mail.nankai.edu.cn}
% \and
% \IEEEauthorblockN{3\textsuperscript{rd} Jiagang Wang}
% \IEEEauthorblockA{\textit{Department of Precision Instruments} \\
% \textit{Tsinghua University}\\
% Beijing, China \\
% 13193093293@163.com}
% \and
% \IEEEauthorblockN{4\textsuperscript{th} Jingyu Wang}
% \IEEEauthorblockA{\textit{College of Software} \\
% \textit{Nankai University}\\
% Tianjin, China \\
% airmonkey2022@outlook.com}
% \and
% \hspace{-2em}\IEEEauthorblockN{5\textsuperscript{th} Yongqian Sun}
% \IEEEauthorblockA{
% \hspace{-2em}\textit{College of Software} \\
% \hspace{-2em}\textit{Nankai University}\\
% \hspace{-2em}Tianjin, China \\
% \hspace{-2em}sunyongqian@nankai.edu.cn}
% \and
% \hspace{-0.5em}\IEEEauthorblockN{6\textsuperscript{th} Xiaolei Hua}
% \IEEEauthorblockA{
% \hspace{-0.5em}\textit{China Mobile Research Institute} \\
% \hspace{-0.5em}\textit{JIUTIAN Team}\\
% \hspace{-0.5em}Beijing, China \\
% \hspace{-0.5em}huaxiaolei@chinamobile.com}
% \and
% \IEEEauthorblockN{7\textsuperscript{th} Lin Zhu}
% \IEEEauthorblockA{
% \textit{China Mobile Research Institute} \\
% \textit{JIUTIAN Team}\\
% Beijing, China \\
% zhulinyj@chinamobile.com}
% \and
% \IEEEauthorblockN{8\textsuperscript{th} Dan Pei}
% \IEEEauthorblockA{\textit{Department of Computer Science} \\
% \textit{Tsinghua University}\\
% Beijing, China \\
% peidan@tsinghua.edu.cn}
% }

% \author{
%     \IEEEauthorblockN{
%     Shenglin Zhang\IEEEauthorrefmark{1}, 
%     Pengtian Zhu\IEEEauthorrefmark{1}, 
%     Jiagang Wang\IEEEauthorrefmark{2}, 
%     Jingyu Wang\IEEEauthorrefmark{1}, \\
%     Yongqian Sun\IEEEauthorrefmark{1}, 
%     Xiaolei Hua\IEEEauthorrefmark{3}, 
%     Lin Zhu\IEEEauthorrefmark{3}, 
%     and Dan Pei\IEEEauthorrefmark{4}
%     } 
    
%     \IEEEauthorblockA{\IEEEauthorrefmark{1}\textit{College of Software},
%     \textit{Nankai University},
%     Tianjin, China}
    
%     \IEEEauthorblockA{\IEEEauthorrefmark{2}\textit{Department of Precision Instruments}, 
%     \textit{Tsinghua University},
%     Beijing, China}
    
%     \IEEEauthorblockA{\IEEEauthorrefmark{3}\textit{JIUTIAN Team},
%     \textit{China Mobile Research Institute},
%     Beijing, China}
    
%     \IEEEauthorblockA{\IEEEauthorrefmark{4}\textit{Department of Computer Science}, 
%     \textit{Tsinghua University},
%     Beijing, China}

%     \IEEEauthorblockA{
%     \{zhangsl,sunyongqian\}@nankai.edu.cn, 
%     zpt@mail.nankai.edu.cn, 
%     13193093293@163.com, \\
%     airmonkey2022@outlook.com, 
%     \{huaxiaolei, zhulinyj\}@chinamobile.com,
%     peidan@tsinghua.edu.cn}
% } 

==> tabs/method_compare.tex <==
\begin{table}[!htb]
\centering
\caption{Comparison of different self-alignment methods.}\label{tab-method-compare}
\resizebox{1.\columnwidth}{!}{
\begin{tabular}{c | c c c c c} 
\hline
{Method} & \makecell[c]{Self \\ Generate Data} & \makecell[c]{Data \\ Privacy} & \makecell[c]{No Human \\ Annotation} & \makecell[c]{Correctness\\Assurance} & \makecell[c]{Iterative\\learning capability}\\ 
\hline
Self-Chat\cite{xu2023baize} & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
Self-Instruct\cite{wang2022self} & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\times$ \\
Self-QA\cite{zhang2023self} & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
Self-Align\cite{sun2024principle} & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
\hline
\textbf{\makecell[c]{Self-Evolution \\ (Our Method)}} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\hline
\end{tabular}}
\end{table}

% \begin{table}[!htb]
% \centering
% \caption{Comparison of different self-alignment methods.}
% \label{Table-compare}
% \resizebox{1.\columnwidth}{!}{
% \begin{tabular}{c | cc cc ccc} 
% \hline
% {Method} & \makecell[c]{No manual\\instructions} & \makecell[c]{Correctness\\assurance} & \makecell[c]{Domain-specific\\guarantee} & \makecell[c]{Iterative\\learning capability}\\ 
% \hline
% Self-Instruct\cite{wang2022self} & $\times$ & $\times$ & $\times$ & $\times$ \\
% Self-Chat\cite{xu2023baize} & $\times$ & $\times$ & $\times$ & $\times$ \\
% Self-Align\cite{sun2024principle} & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ \\
% Self-QA\cite{zhang2023self} & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ \\
% \hline
% \textbf{Self-Evolution} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
% \hline
% \end{tabular}}
% \end{table}
